Zero-Shot Prompting Approaches for LLM-based Graphical User Interface Generation

Graphical user interface (GUI) prototyping represents an essential activity in the development of interactive systems, which are omnipresent today. GUI prototypes facilitate elicitation of requirements and help to test, evaluate, and validate ideas with users and the development team. However, creating GUI prototypes is a time-consuming process and often requires extensive resources. While existing research for automatic GUI generation focused largely on resource-intensive training and fine-tuning of LLMs, mainly for low-fidelity GUIs, we investigate the potential and effectiveness of Zero-Shot (ZS) prompting for high-fidelity GUI generation. We propose a Retrieval-Augmented GUI Generation (RAGG) approach, integrated with an LLM-based GUI retrieval re-ranking and filtering mechanism based on a large-scale GUI repository. In addition, we adapt Prompt Decomposition (PDGG) and Self-Critique (SCGG) for GUI generation. To evaluate the effectiveness of the proposed ZS prompting approaches for GUI generation, we extensively evaluated the accuracy and subjective satisfaction of the generated GUI prototypes. Our evaluation, which encompasses over 3,000 GUI annotations from over 100 crowd-workers with UI/UX experience, shows that SCGG, in contrast to PDGG and RAGG, can lead to more effective GUI generation, and provides valuable insights into the defects that are produced by the LLMs in the generated GUI prototypes.

==> chapters/backup.tex <==
\begin{table}[h]
\caption{p-Values (Wilcoxon Signed-Rank Test) for different SCGG loops and eight evaluated aspects (N=150). A: \textit{Feature Cover.}, B: \textit{Feature Width}, C: \textit{Feature Impl.}, D: \textit{Inform. Organization}, E: \textit{Appealing Design}, F: \textit{Minimal Errors}, G: \textit{Overall Satisfied}, H: \textit{Complete App}.}
\label{tab:results_scgg_k}
\centering
\small
\begin{tabular}{|c|ll|ll|ll|}
\hline 
\rule{0pt}{2.2ex} 
\textbf{loop}  & \multicolumn{2}{c|}{\textbf{2}} & \multicolumn{2}{c|}{\textbf{3}} & \multicolumn{2}{c|}{\textbf{4}} \\ \hline \hline
\textbf{\begin{tabular}[c]{@{}c@{}}\textbf{1}\end{tabular}} & \cellcolor[HTML]{F5F5F5}\begin{tabular}[c]{@{}l@{}}
\scriptsize .497 (A)\\ 
\scriptsize \textbf{.000} (B)\\ 
\scriptsize .365 (C)\\ 
\scriptsize .164 (D)\end{tabular} & \begin{tabular}[c]{@{}l@{}}
\scriptsize .064 (E)\\ 
\scriptsize .743 (F)\\ 
\scriptsize .194 (G)\\ 
\scriptsize \textbf{.002} (H)\end{tabular} & \cellcolor[HTML]{F5F5F5}\begin{tabular}[c]{@{}l@{}}
\scriptsize .536 (A)\\ 
\scriptsize \textbf{.000} (B)\\ 
\scriptsize .398 (C)\\ 
\scriptsize .495 (D)\end{tabular} & \begin{tabular}[c]{@{}l@{}}
\scriptsize .085 (E)\\ 
\scriptsize .650 (F)\\ 
\scriptsize .073 (G)\\ 
\scriptsize \textbf{.012} (H)\end{tabular} & \cellcolor[HTML]{F5F5F5}\begin{tabular}[c]{@{}l@{}}
\scriptsize .704 (A)\\ 
\scriptsize \textbf{.000} (B)\\ 
\scriptsize .503 (C)\\ 
\scriptsize .532 (D)\end{tabular} & \begin{tabular}[c]{@{}l@{}}
\scriptsize .384 (E)\\ 
\scriptsize .292 (F)\\ 
\scriptsize .658 (G)\\ 
\scriptsize .304 (H)\end{tabular} \\ \hline \hline
\begin{tabular}[c]{@{}c@{}}\textbf{2}\end{tabular} & \cellcolor[HTML]{F5F5F5} &  & \cellcolor[HTML]{F5F5F5}\begin{tabular}[c]{@{}l@{}}
\scriptsize .923 (A)\\ 
\scriptsize .094 (B)\\ 
\scriptsize .953 (C)\\ 
\scriptsize .575 (D)\end{tabular} & \begin{tabular}[c]{@{}l@{}}
\scriptsize .876 (E)\\ 
\scriptsize .999 (F)\\ 
\scriptsize .519 (G)\\ 
\scriptsize .606 (H)\end{tabular} & \cellcolor[HTML]{F5F5F5}\begin{tabular}[c]{@{}l@{}}

\scriptsize .810 (A)\\ 
\scriptsize .159 (B)\\ 
\scriptsize .848 (C)\\ 
\scriptsize .091 (D)\end{tabular} & \begin{tabular}[c]{@{}l@{}}
\scriptsize .294 (E)\\ 
\scriptsize .404 (F)\\ 
\scriptsize .296 (G)\\ 
\scriptsize \textbf{.033} (H)\end{tabular} \\ \hline \hline
\textbf{\begin{tabular}[c]{@{}c@{}}\textbf{3}\end{tabular}} & \cellcolor[HTML]{F5F5F5} &  & \cellcolor[HTML]{F5F5F5} &  & \cellcolor[HTML]{F5F5F5}\begin{tabular}[c]{@{}l@{}}
\scriptsize .930 (A)\\ 
\scriptsize .969 (B)\\ 
\scriptsize .926 (C)\\ 
\scriptsize .222 (D)\end{tabular} & \begin{tabular}[c]{@{}l@{}}
\scriptsize .488 (E)\\ 
\scriptsize .618 (F)\\ 
\scriptsize .150 (G)\\ 
\scriptsize .111 (H)\end{tabular} \\ \hline
\end{tabular}
\end{table}
